Maximum entropy methods for texture synthesis: theory and practice

Recent years have seen the rise of convolutional neural network techniques in exemplar-based image synthesis. These methods often rely on the minimization of some variational formulation on the image space for which the minimizers are assumed to be the solutions of the synthesis problem. In this paper we investigate, both theoretically and experimentally, another framework to deal with this problem using an alternate sampling/minimization scheme. First, we use results from information geometry to assess that our method yields a probability measure which has maximum entropy under some constraints in expectation. Then, we turn to the analysis of our method and we show, using recent results from the Markov chain literature, that its error can be explicitly bounded with constants which depend polynomially in the dimension even in the non-convex setting. This includes the case where the constraints are defined via a differentiable neural network. Finally, we present an extensive experimental study of the model, including a comparison with state-of-the-art methods and an extension to style transfer.

==> behavior_parameter.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> data/sweet_w_03_00.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, 75.445656) 
(11900, 70.65666) 
(12900, 65.57581) 
(13900, 59.887096) 
(14900, 53.551773) 
(15900, 46.332) 
(16900, 37.57846) 
(17900, 29.111584) 
(18900, 19.810146) 
(19900, 9.681523) 
(20900, -0.67518497) 
(21900, -13.150966) 
(22900, -20.865068) 
(23900, -25.334332) 
(24900, -32.8285) 
(25900, -42.350086) 
(26900, -54.4982) 
(27900, -66.41157) 
(28900, -79.669495) 
(29900, -90.95275) 
(30900, -101.74959) 
(31900, -112.68143) 
(32900, -125.20874) 
(33900, -136.66168) 
(34900, -149.05212) 
(35900, -159.56471) 
(36900, -170.78482) 
(37900, -183.12807) 
(38900, -195.31146) 
(39900, -209.95303) 
(40900, -224.16165) 
(41900, -238.03127) 
(42900, -251.44582) 
(43900, -264.42273) 
(44900, -277.26526) 
(45900, -291.09604) 
(46900, -303.66064) 
(47900, -318.59912) 
(48900, -331.64893) 
(49900, -346.64044) 
(50900, -361.62817) 
(51900, -378.053) 
(52900, -392.0252) 
(53900, -404.23358) 
(54900, -418.82855) 
(55900, -433.827) 
(56900, -447.35364) 
(57900, -461.37823) 
(58900, -474.49017) 
(59900, -489.3306) 
(60900, -503.4612) 
(61900, -519.2265) 
(62900, -535.0735) 
(63900, -550.45056) 
(64900, -563.21906) 
(65900, -577.4044) 
(66900, -591.41797) 
(67900, -604.6735) 
(68900, -618.62085) 
(69900, -632.21375) 
(70900, -646.3005) 
(71900, -660.28705) 
(72900, -673.66656) 
(73900, -687.39594) 
(74900, -701.4143) 
(75900, -712.94366) 
(76900, -726.7508) 
(77900, -740.16223) 
(78900, -755.1625) 
(79900, -771.2055) 
(80900, -786.7474) 
(81900, -802.23083) 
(82900, -816.8361) 
(83900, -832.5547) 
(84900, -847.3693) 
(85900, -864.7208) 
(86900, -881.1848) 
(87900, -898.6979) 
(88900, -916.1592) 
(89900, -932.7364) 
(90900, -950.2861) 
(91900, -967.446) 
(92900, -983.8053) 
(93900, -1000.64606) 
(94900, -1018.2591) 
(95900, -1034.6224) 
(96900, -1052.3336) 
(97900, -1068.7505) 
(98900, -1084.8026) 
(99900, -1100.6232) 
};

==> data/sweet_w_03_10.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, 799.12213) 
(11900, 842.243) 
(12900, 886.69604) 
(13900, 931.58325) 
(14900, 973.96643) 
(15900, 1011.6687) 
(16900, 1046.8448) 
(17900, 1079.9106) 
(18900, 1112.1498) 
(19900, 1143.0184) 
(20900, 1170.4974) 
(21900, 1196.5139) 
(22900, 1225.8198) 
(23900, 1254.7512) 
(24900, 1277.776) 
(25900, 1298.4214) 
(26900, 1317.1501) 
(27900, 1338.1785) 
(28900, 1360.5101) 
(29900, 1381.7185) 
(30900, 1403.5852) 
(31900, 1424.8951) 
(32900, 1445.2253) 
(33900, 1467.1869) 
(34900, 1489.3398) 
(35900, 1511.1827) 
(36900, 1531.497) 
(37900, 1552.9623) 
(38900, 1572.4342) 
(39900, 1594.437) 
(40900, 1614.6414) 
(41900, 1633.6713) 
(42900, 1653.7396) 
(43900, 1674.0006) 
(44900, 1693.5586) 
(45900, 1713.3151) 
(46900, 1732.777) 
(47900, 1749.0364) 
(48900, 1767.7255) 
(49900, 1783.1613) 
(50900, 1798.2887) 
(51900, 1811.912) 
(52900, 1826.542) 
(53900, 1840.5652) 
(54900, 1854.771) 
(55900, 1871.7662) 
(56900, 1886.3196) 
(57900, 1901.8629) 
(58900, 1917.4231) 
(59900, 1933.9666) 
(60900, 1951.3145) 
(61900, 1965.9528) 
(62900, 1980.4445) 
(63900, 1995.8077) 
(64900, 2011.032) 
(65900, 2026.9836) 
(66900, 2042.3763) 
(67900, 2058.1145) 
(68900, 2071.9583) 
(69900, 2087.5977) 
(70900, 2101.603) 
(71900, 2115.8198) 
(72900, 2128.5283) 
(73900, 2141.1096) 
(74900, 2155.8457) 
(75900, 2170.2695) 
(76900, 2183.5686) 
(77900, 2196.351) 
(78900, 2209.1782) 
(79900, 2221.0457) 
(80900, 2232.9482) 
(81900, 2245.5134) 
(82900, 2260.791) 
(83900, 2274.5789) 
(84900, 2288.3274) 
(85900, 2300.5144) 
(86900, 2312.672) 
(87900, 2323.6543) 
(88900, 2336.3784) 
(89900, 2347.8955) 
(90900, 2359.7588) 
(91900, 2370.7961) 
(92900, 2382.3545) 
(93900, 2393.416) 
(94900, 2404.4727) 
(95900, 2415.9343) 
(96900, 2427.8508) 
(97900, 2440.5535) 
(98900, 2452.7278) 
(99900, 2463.6538) 
};

==> data/sweet_w_03_20.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, 678.78516) 
(11900, 716.92896) 
(12900, 753.5953) 
(13900, 787.7948) 
(14900, 822.0515) 
(15900, 854.0691) 
(16900, 883.75995) 
(17900, 912.0729) 
(18900, 939.0478) 
(19900, 966.6042) 
(20900, 992.35693) 
(21900, 1017.1012) 
(22900, 1044.6653) 
(23900, 1067.5422) 
(24900, 1081.2067) 
(25900, 1098.1694) 
(26900, 1111.6873) 
(27900, 1127.7523) 
(28900, 1140.2844) 
(29900, 1153.701) 
(30900, 1166.5183) 
(31900, 1176.6453) 
(32900, 1186.8844) 
(33900, 1197.6669) 
(34900, 1207.8474) 
(35900, 1219.6145) 
(36900, 1230.8187) 
(37900, 1244.9045) 
(38900, 1255.9885) 
(39900, 1267.9047) 
(40900, 1280.2258) 
(41900, 1290.8864) 
(42900, 1303.6866) 
(43900, 1312.5382) 
(44900, 1324.5621) 
(45900, 1335.4011) 
(46900, 1346.7554) 
(47900, 1354.8899) 
(48900, 1367.7328) 
(49900, 1378.2673) 
(50900, 1390.5631) 
(51900, 1401.5114) 
(52900, 1412.0358) 
(53900, 1422.2878) 
(54900, 1432.5089) 
(55900, 1444.7114) 
(56900, 1454.8022) 
(57900, 1464.5245) 
(58900, 1474.8281) 
(59900, 1483.3314) 
(60900, 1493.0933) 
(61900, 1501.2422) 
(62900, 1507.1493) 
(63900, 1515.6399) 
(64900, 1526.8243) 
(65900, 1537.5854) 
(66900, 1546.9674) 
(67900, 1556.266) 
(68900, 1565.6539) 
(69900, 1576.4719) 
(70900, 1584.4125) 
(71900, 1594.296) 
(72900, 1605.6237) 
(73900, 1616.7924) 
(74900, 1627.1882) 
(75900, 1637.2659) 
(76900, 1646.5112) 
(77900, 1654.6818) 
(78900, 1662.7383) 
(79900, 1669.6807) 
(80900, 1677.12) 
(81900, 1686.6542) 
(82900, 1693.7338) 
(83900, 1701.4304) 
(84900, 1711.5898) 
(85900, 1720.5183) 
(86900, 1729.9119) 
(87900, 1737.2726) 
(88900, 1743.4435) 
(89900, 1750.2915) 
(90900, 1756.1637) 
(91900, 1761.1372) 
(92900, 1767.5155) 
(93900, 1772.8947) 
(94900, 1777.7825) 
(95900, 1782.4513) 
(96900, 1785.9266) 
(97900, 1792.1846) 
(98900, 1799.1345) 
(99900, 1806.6873) 
};

==> data/sweet_w_08_00.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, 297.31265) 
(11900, 291.55902) 
(12900, 278.7522) 
(13900, 257.12076) 
(14900, 242.69664) 
(15900, 238.37071) 
(16900, 233.80101) 
(17900, 231.66762) 
(18900, 227.06906) 
(19900, 223.48318) 
(20900, 226.96628) 
(21900, 218.26723) 
(22900, 225.18939) 
(23900, 211.28381) 
(24900, 236.66089) 
(25900, 253.1019) 
(26900, 264.6494) 
(27900, 269.28806) 
(28900, 272.89844) 
(29900, 272.9772) 
(30900, 280.98782) 
(31900, 279.53632) 
(32900, 278.54074) 
(33900, 268.66238) 
(34900, 261.07452) 
(35900, 271.2239) 
(36900, 276.7892) 
(37900, 270.46033) 
(38900, 266.65704) 
(39900, 273.76773) 
(40900, 283.01987) 
(41900, 296.41492) 
(42900, 304.53943) 
(43900, 306.73492) 
(44900, 315.11655) 
(45900, 312.9479) 
(46900, 311.1472) 
(47900, 312.35178) 
(48900, 317.09885) 
(49900, 310.72687) 
(50900, 300.30515) 
(51900, 302.14026) 
(52900, 291.51526) 
(53900, 285.9419) 
(54900, 278.89978) 
(55900, 272.34055) 
(56900, 273.27426) 
(57900, 268.92746) 
(58900, 265.82547) 
(59900, 249.84766) 
(60900, 248.23207) 
(61900, 256.09262) 
(62900, 260.30756) 
(63900, 268.70514) 
(64900, 265.37738) 
(65900, 264.9135) 
(66900, 269.5605) 
(67900, 274.9258) 
(68900, 279.13193) 
(69900, 283.38678) 
(70900, 282.2485) 
(71900, 280.80484) 
(72900, 276.01483) 
(73900, 279.9774) 
(74900, 287.1398) 
(75900, 287.08212) 
(76900, 287.37756) 
(77900, 293.37784) 
(78900, 298.2484) 
(79900, 299.31226) 
(80900, 293.0326) 
(81900, 293.63297) 
(82900, 300.53506) 
(83900, 305.52194) 
(84900, 312.29846) 
(85900, 315.3805) 
(86900, 315.96375) 
(87900, 318.01587) 
(88900, 333.7198) 
(89900, 334.67795) 
(90900, 336.39117) 
(91900, 333.55606) 
(92900, 331.15866) 
(93900, 327.16858) 
(94900, 324.96) 
(95900, 319.0961) 
(96900, 312.89716) 
(97900, 312.21317) 
(98900, 323.85507) 
(99900, 327.57794) 
};

==> data/sweet_w_08_10.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, -181.4394) 
(11900, -178.11942) 
(12900, -170.63507) 
(13900, -167.66447) 
(14900, -152.3882) 
(15900, -145.46552) 
(16900, -133.0165) 
(17900, -115.327415) 
(18900, -122.78783) 
(19900, -115.48013) 
(20900, -111.12954) 
(21900, -108.116554) 
(22900, -88.00993) 
(23900, -102.931076) 
(24900, -100.93226) 
(25900, -106.50962) 
(26900, -118.69347) 
(27900, -117.624245) 
(28900, -130.51369) 
(29900, -153.85976) 
(30900, -148.99503) 
(31900, -154.35725) 
(32900, -157.12859) 
(33900, -157.98515) 
(34900, -172.11563) 
(35900, -173.0584) 
(36900, -171.32513) 
(37900, -161.15729) 
(38900, -158.6769) 
(39900, -151.14545) 
(40900, -152.60144) 
(41900, -155.40721) 
(42900, -158.70428) 
(43900, -162.41531) 
(44900, -160.23041) 
(45900, -173.12875) 
(46900, -178.01474) 
(47900, -186.78253) 
(48900, -180.17795) 
(49900, -173.38266) 
(50900, -166.16022) 
(51900, -175.40143) 
(52900, -183.24785) 
(53900, -180.9278) 
(54900, -190.56093) 
(55900, -185.89288) 
(56900, -192.83722) 
(57900, -190.21338) 
(58900, -195.13618) 
(59900, -203.9573) 
(60900, -212.17004) 
(61900, -208.63394) 
(62900, -215.5251) 
(63900, -210.47592) 
(64900, -207.55441) 
(65900, -197.78326) 
(66900, -207.36578) 
(67900, -213.03929) 
(68900, -218.71019) 
(69900, -221.75288) 
(70900, -218.14117) 
(71900, -225.23267) 
(72900, -233.3503) 
(73900, -226.53296) 
(74900, -226.8603) 
(75900, -224.89964) 
(76900, -234.11972) 
(77900, -224.1317) 
(78900, -223.10838) 
(79900, -214.24991) 
(80900, -208.41565) 
(81900, -208.65747) 
(82900, -218.57916) 
(83900, -213.68134) 
(84900, -198.77484) 
(85900, -200.15332) 
(86900, -187.1232) 
(87900, -186.01471) 
(88900, -187.13516) 
(89900, -179.0134) 
(90900, -183.61644) 
(91900, -195.21022) 
(92900, -198.92438) 
(93900, -200.51848) 
(94900, -205.51941) 
(95900, -210.75583) 
(96900, -221.62013) 
(97900, -212.04204) 
(98900, -204.75493) 
(99900, -193.6743) 
};

==> data/sweet_w_08_20.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, 101.60741) 
(11900, 93.718094) 
(12900, 91.47624) 
(13900, 78.924866) 
(14900, 93.56206) 
(15900, 113.06424) 
(16900, 122.89473) 
(17900, 131.0811) 
(18900, 134.41312) 
(19900, 130.8814) 
(20900, 134.43071) 
(21900, 131.27695) 
(22900, 129.59067) 
(23900, 138.12738) 
(24900, 149.90651) 
(25900, 130.08789) 
(26900, 135.4886) 
(27900, 147.14638) 
(28900, 175.94702) 
(29900, 195.87839) 
(30900, 212.57326) 
(31900, 212.32635) 
(32900, 227.40428) 
(33900, 226.1924) 
(34900, 220.16406) 
(35900, 212.82437) 
(36900, 222.12456) 
(37900, 231.11368) 
(38900, 231.65662) 
(39900, 225.24977) 
(40900, 221.69748) 
(41900, 215.36328) 
(42900, 213.78514) 
(43900, 202.74297) 
(44900, 203.61816) 
(45900, 210.83463) 
(46900, 223.5346) 
(47900, 227.17711) 
(48900, 230.27528) 
(49900, 225.95546) 
(50900, 233.78745) 
(51900, 233.50864) 
(52900, 229.06491) 
(53900, 230.00914) 
(54900, 233.79932) 
(55900, 240.62456) 
(56900, 250.50414) 
(57900, 256.83994) 
(58900, 266.18008) 
(59900, 258.356) 
(60900, 255.64781) 
(61900, 253.02649) 
(62900, 240.5728) 
(63900, 232.91388) 
(64900, 237.62105) 
(65900, 247.02611) 
(66900, 255.71599) 
(67900, 257.30533) 
(68900, 248.2569) 
(69900, 234.35443) 
(70900, 225.62924) 
(71900, 219.94034) 
(72900, 225.37573) 
(73900, 221.45784) 
(74900, 216.48175) 
(75900, 223.75018) 
(76900, 231.80557) 
(77900, 237.20854) 
(78900, 237.97737) 
(79900, 232.7878) 
(80900, 233.42924) 
(81900, 242.10155) 
(82900, 245.97536) 
(83900, 235.71826) 
(84900, 243.4769) 
(85900, 249.24467) 
(86900, 258.6391) 
(87900, 253.92606) 
(88900, 251.48402) 
(89900, 258.58472) 
(90900, 255.87344) 
(91900, 246.26611) 
(92900, 238.1005) 
(93900, 240.82329) 
(94900, 240.88475) 
(95900, 236.76625) 
(96900, 231.95718) 
(97900, 233.92607) 
(98900, 232.56879) 
(99900, 229.66498) 
};

==> data/sweet_w_24_00.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, -43.12973) 
(11900, -28.442026) 
(12900, -58.88528) 
(13900, -51.242897) 
(14900, -51.399734) 
(15900, -14.026662) 
(16900, -10.313433) 
(17900, -39.83258) 
(18900, -29.510904) 
(19900, -13.8111725) 
(20900, -4.0295906) 
(21900, -7.564149) 
(22900, -56.926094) 
(23900, -44.96322) 
(24900, -55.837505) 
(25900, -64.40076) 
(26900, -12.298994) 
(27900, -18.589928) 
(28900, -32.367416) 
(29900, -15.503866) 
(30900, -36.381283) 
(31900, -27.376259) 
(32900, -41.139736) 
(33900, -10.91538) 
(34900, -1.2003653) 
(35900, -19.919834) 
(36900, -18.075752) 
(37900, -27.356903) 
(38900, -31.651903) 
(39900, -6.176399) 
(40900, -0.21475708) 
(41900, -26.436878) 
(42900, -24.305038) 
(43900, -20.4409) 
(44900, -10.086509) 
(45900, -30.541159) 
(46900, -8.871135) 
(47900, -22.459475) 
(48900, 5.956434) 
(49900, -10.933387) 
(50900, -5.458145) 
(51900, 2.625892) 
(52900, -4.059069) 
(53900, -10.116113) 
(54900, -29.573559) 
(55900, -5.978237) 
(56900, -23.602503) 
(57900, -12.73037) 
(58900, -26.611757) 
(59900, -21.377768) 
(60900, -17.910034) 
(61900, 0.36605996) 
(62900, -17.350283) 
(63900, -14.002037) 
(64900, 6.6374893) 
(65900, -2.3130145) 
(66900, 3.6611395) 
(67900, 9.303107) 
(68900, 0.3560007) 
(69900, -19.806519) 
(70900, -17.869871) 
(71900, -16.115324) 
(72900, -24.026161) 
(73900, -22.061348) 
(74900, -20.941462) 
(75900, -20.358442) 
(76900, -12.654279) 
(77900, -28.966959) 
(78900, -4.290872) 
(79900, 0.7373839) 
(80900, -13.893942) 
(81900, -22.360264) 
(82900, -3.1453066) 
(83900, -7.939608) 
(84900, -4.455418) 
(85900, 12.162724) 
(86900, -9.7807) 
(87900, 2.9423327) 
(88900, 1.2201556) 
(89900, -0.726406) 
(90900, -8.532127) 
(91900, -21.487629) 
(92900, -9.182962) 
(93900, -17.417372) 
(94900, -14.641602) 
(95900, -13.513178) 
(96900, -32.980324) 
(97900, -30.642776) 
(98900, -11.4409275) 
(99900, -35.308384) 
};

==> data/sweet_w_24_10.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, -2.7167637) 
(11900, -11.288211) 
(12900, -12.851279) 
(13900, -12.400504) 
(14900, 12.361622) 
(15900, 6.0868554) 
(16900, 0.84569657) 
(17900, 5.6256847) 
(18900, 13.265278) 
(19900, 12.011822) 
(20900, 7.928706) 
(21900, -0.8354347) 
(22900, 9.875683) 
(23900, 27.503197) 
(24900, -35.92533) 
(25900, 5.5198364) 
(26900, 18.10809) 
(27900, -13.709347) 
(28900, -4.72393) 
(29900, 0.50597197) 
(30900, 13.188585) 
(31900, 19.789816) 
(32900, -9.278195) 
(33900, 13.103058) 
(34900, -7.9627185) 
(35900, 9.751884) 
(36900, 11.8707) 
(37900, -3.2603848) 
(38900, 0.27532202) 
(39900, -8.975449) 
(40900, -9.582744) 
(41900, 9.8136215) 
(42900, 2.2790902) 
(43900, 18.032167) 
(44900, -4.062137) 
(45900, 1.3096516) 
(46900, -6.7276115) 
(47900, 3.6556823) 
(48900, -2.6608164) 
(49900, 15.081979) 
(50900, -6.229713) 
(51900, 18.19915) 
(52900, 0.5148229) 
(53900, 3.2579906) 
(54900, 8.926146) 
(55900, 8.9828615) 
(56900, 5.3126564) 
(57900, 7.66527) 
(58900, -0.12307911) 
(59900, 7.247756) 
(60900, 5.600228) 
(61900, 5.9659433) 
(62900, 12.568241) 
(63900, 21.482038) 
(64900, 9.283465) 
(65900, 23.43427) 
(66900, 3.8090785) 
(67900, 2.3327706) 
(68900, -4.2631097) 
(69900, -23.367819) 
(70900, -10.570477) 
(71900, -15.210691) 
(72900, -11.286558) 
(73900, -22.382944) 
(74900, -6.522945) 
(75900, 3.0539331) 
(76900, -21.658257) 
(77900, -8.968987) 
(78900, -17.726627) 
(79900, -7.8489623) 
(80900, -15.210676) 
(81900, -9.771029) 
(82900, -13.278338) 
(83900, -12.5826435) 
(84900, -14.12741) 
(85900, -9.144086) 
(86900, -13.520155) 
(87900, -4.096535) 
(88900, 1.2816099) 
(89900, -1.3551165) 
(90900, -2.3313618) 
(91900, -2.4364839) 
(92900, -6.265231) 
(93900, -17.080183) 
(94900, -2.0624242) 
(95900, -0.60773623) 
(96900, -18.892149) 
(97900, -8.369508) 
(98900, -8.542733) 
(99900, 4.9480243) 
};

==> data/sweet_w_24_20.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, 39.533577) 
(11900, 7.9136496) 
(12900, 39.184746) 
(13900, 31.360205) 
(14900, 29.30167) 
(15900, 48.165806) 
(16900, 39.721756) 
(17900, 50.170826) 
(18900, 28.299416) 
(19900, 21.47716) 
(20900, 23.10791) 
(21900, 8.395138) 
(22900, 24.759949) 
(23900, 33.20483) 
(24900, 25.185678) 
(25900, 15.475697) 
(26900, -4.657378) 
(27900, 10.045404) 
(28900, 13.345047) 
(29900, 13.983602) 
(30900, 23.080215) 
(31900, 18.157671) 
(32900, 21.505186) 
(33900, 15.856339) 
(34900, 18.855253) 
(35900, 26.130527) 
(36900, 24.555721) 
(37900, 29.542406) 
(38900, -1.0551391) 
(39900, 7.9478397) 
(40900, -3.3656113) 
(41900, 9.087456) 
(42900, -4.257847) 
(43900, 16.958317) 
(44900, 17.006218) 
(45900, 8.174538) 
(46900, -4.0000978) 
(47900, 1.3997513) 
(48900, 13.52263) 
(49900, 8.325446) 
(50900, -7.0703664) 
(51900, 1.2497032) 
(52900, -2.0751104) 
(53900, -1.4308672) 
(54900, -12.186948) 
(55900, 9.942021) 
(56900, 0.40264922) 
(57900, 6.3987746) 
(58900, -13.397561) 
(59900, 3.817218) 
(60900, -0.28333098) 
(61900, 6.9412274) 
(62900, 5.4954805) 
(63900, -6.6263924) 
(64900, -5.764934) 
(65900, 9.203571) 
(66900, 18.416838) 
(67900, 28.258543) 
(68900, 10.731571) 
(69900, 20.32842) 
(70900, -6.621127) 
(71900, 0.40968227) 
(72900, -6.8111324) 
(73900, 13.225327) 
(74900, 3.8693678) 
(75900, -14.25133) 
(76900, -6.2569847) 
(77900, -9.513511) 
(78900, -0.24011713) 
(79900, 7.2613964) 
(80900, 13.312194) 
(81900, 17.163124) 
(82900, 17.389223) 
(83900, -2.6010227) 
(84900, 19.098278) 
(85900, 10.453601) 
(86900, -1.5262402) 
(87900, -12.35151) 
(88900, -7.386893) 
(89900, 8.245576) 
(90900, 1.9464065) 
(91900, 8.87803) 
(92900, 4.6031566) 
(93900, 8.491642) 
(94900, -4.913677) 
(95900, -2.3251555) 
(96900, 1.9524121) 
(97900, -8.588192) 
(98900, -6.140838) 
(99900, -7.7547226) 
};

==> data/sweet_w_31_00.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, 17.194098) 
(11900, 14.257704) 
(12900, 15.891557) 
(13900, 5.0862746) 
(14900, 22.108057) 
(15900, 17.434225) 
(16900, 11.887576) 
(17900, 10.839465) 
(18900, -0.8871777) 
(19900, 18.857662) 
(20900, 17.776123) 
(21900, 9.865712) 
(22900, 14.874124) 
(23900, 4.2313128) 
(24900, 24.666204) 
(25900, 0.45735896) 
(26900, -13.137943) 
(27900, 1.5998065) 
(28900, 1.2496748) 
(29900, 24.85581) 
(30900, 5.881722) 
(31900, 10.833788) 
(32900, 12.961767) 
(33900, 23.078503) 
(34900, 6.3437757) 
(35900, 20.70222) 
(36900, 25.595732) 
(37900, 9.70173) 
(38900, 12.614825) 
(39900, 40.207573) 
(40900, 33.623585) 
(41900, -0.098196745) 
(42900, 23.239809) 
(43900, 33.40362) 
(44900, 27.73659) 
(45900, 13.484123) 
(46900, 30.469969) 
(47900, 18.556684) 
(48900, 0.833297) 
(49900, 32.08649) 
(50900, 11.234545) 
(51900, -4.5387836) 
(52900, -1.4384167) 
(53900, 3.3903556) 
(54900, -3.5447078) 
(55900, 26.978907) 
(56900, -2.9386177) 
(57900, -3.6351256) 
(58900, 28.309242) 
(59900, -2.0039334) 
(60900, 18.23676) 
(61900, -16.396494) 
(62900, 8.140854) 
(63900, -9.342585) 
(64900, -19.874346) 
(65900, 16.224113) 
(66900, -1.9761059) 
(67900, -14.298044) 
(68900, 8.282209) 
(69900, -17.999155) 
(70900, 5.982846) 
(71900, -5.319401) 
(72900, -24.866917) 
(73900, -8.023853) 
(74900, -8.757524) 
(75900, 8.835914) 
(76900, -15.580619) 
(77900, 25.420723) 
(78900, 0.49313903) 
(79900, -4.5164967) 
(80900, -2.0662112) 
(81900, -6.1602426) 
(82900, -20.137213) 
(83900, -0.46832943) 
(84900, -3.454995) 
(85900, -9.656858) 
(86900, 10.018216) 
(87900, -6.229424) 
(88900, 4.0224495) 
(89900, -5.746136) 
(90900, -6.895462) 
(91900, 7.4973173) 
(92900, -4.5307097) 
(93900, 9.675535) 
(94900, -17.431469) 
(95900, -20.99984) 
(96900, -9.349629) 
(97900, 3.6224968) 
(98900, -25.604935) 
(99900, -29.314247) 
};

==> data/sweet_w_31_10.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, -13.503996) 
(11900, -8.058977) 
(12900, -2.5578656) 
(13900, -15.070178) 
(14900, -47.45717) 
(15900, -27.514914) 
(16900, -34.35482) 
(17900, -23.156078) 
(18900, -21.824795) 
(19900, -21.790092) 
(20900, -6.9853544) 
(21900, -10.663893) 
(22900, -9.562104) 
(23900, -18.238266) 
(24900, -9.097354) 
(25900, -18.942379) 
(26900, -9.012409) 
(27900, -16.096115) 
(28900, -21.642916) 
(29900, -6.7856627) 
(30900, -19.693504) 
(31900, 8.452283) 
(32900, -13.773347) 
(33900, 10.364036) 
(34900, 10.927705) 
(35900, -3.3882232) 
(36900, 5.4036303) 
(37900, 2.3288085) 
(38900, -3.4333735) 
(39900, -3.3885095) 
(40900, 5.137828) 
(41900, -6.4586954) 
(42900, -25.267853) 
(43900, -29.593287) 
(44900, -21.835155) 
(45900, -25.994265) 
(46900, -25.737215) 
(47900, -17.35885) 
(48900, -31.806173) 
(49900, -21.84819) 
(50900, -16.825867) 
(51900, -12.703069) 
(52900, -37.07004) 
(53900, -25.500622) 
(54900, -19.507332) 
(55900, -36.192158) 
(56900, -20.62919) 
(57900, -21.818066) 
(58900, -4.900424) 
(59900, -19.175787) 
(60900, -26.756907) 
(61900, -17.088463) 
(62900, -23.21139) 
(63900, -38.681015) 
(64900, -28.355803) 
(65900, -43.501568) 
(66900, -48.981236) 
(67900, -49.138992) 
(68900, -55.58543) 
(69900, -35.982624) 
(70900, -36.87934) 
(71900, -45.682987) 
(72900, -46.833813) 
(73900, -47.7449) 
(74900, -42.299942) 
(75900, -45.008255) 
(76900, -12.181101) 
(77900, -22.856579) 
(78900, -31.46582) 
(79900, -17.726072) 
(80900, -14.738777) 
(81900, -13.1086645) 
(82900, -22.608881) 
(83900, -28.02308) 
(84900, -37.782024) 
(85900, -21.186483) 
(86900, -17.931843) 
(87900, -29.93013) 
(88900, -22.351957) 
(89900, -28.674442) 
(90900, -30.51082) 
(91900, -11.026972) 
(92900, -15.598172) 
(93900, -20.841751) 
(94900, -25.780544) 
(95900, -37.380978) 
(96900, -33.823086) 
(97900, -13.4816) 
(98900, -37.341232) 
(99900, -19.604223) 
};

==> data/sweet_w_31_20.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, 27.03161) 
(11900, 19.642391) 
(12900, 19.74116) 
(13900, 44.706806) 
(14900, 32.29954) 
(15900, 18.12128) 
(16900, 29.800846) 
(17900, 18.965895) 
(18900, 28.429686) 
(19900, 26.052132) 
(20900, 31.377892) 
(21900, 34.6953) 
(22900, 39.496685) 
(23900, 1.0578245) 
(24900, -0.39662918) 
(25900, 13.065274) 
(26900, 17.68791) 
(27900, -5.512599) 
(28900, 3.9367986) 
(29900, 2.234136) 
(30900, -1.1909688) 
(31900, 2.9561276) 
(32900, -8.793632) 
(33900, 12.533424) 
(34900, 6.530412) 
(35900, 7.6936088) 
(36900, 15.7140665) 
(37900, 13.934894) 
(38900, 4.618345) 
(39900, -10.033042) 
(40900, -3.2928755) 
(41900, 23.468416) 
(42900, 9.703652) 
(43900, 6.3787827) 
(44900, 1.8683611) 
(45900, -7.0847487) 
(46900, 3.8589509) 
(47900, 0.5517846) 
(48900, -2.8154366) 
(49900, 4.1936574) 
(50900, 13.482409) 
(51900, 2.668105) 
(52900, 11.022691) 
(53900, 7.7637568) 
(54900, 25.681189) 
(55900, -5.4031706) 
(56900, 12.550924) 
(57900, 15.639463) 
(58900, 10.360761) 
(59900, 2.82774) 
(60900, -1.5475553) 
(61900, 8.610865) 
(62900, 9.559555) 
(63900, 25.946587) 
(64900, 6.174591) 
(65900, 9.852377) 
(66900, 9.261679) 
(67900, 16.898062) 
(68900, 11.783463) 
(69900, 5.974927) 
(70900, 9.244666) 
(71900, 24.175583) 
(72900, 27.757954) 
(73900, 4.333374) 
(74900, 9.822105) 
(75900, 9.718816) 
(76900, 19.80594) 
(77900, 6.1607156) 
(78900, 14.422527) 
(79900, 1.1053102) 
(80900, 0.1824545) 
(81900, -0.342205) 
(82900, 5.372636) 
(83900, 6.9731665) 
(84900, 19.969284) 
(85900, 21.93079) 
(86900, 33.300385) 
(87900, 17.626217) 
(88900, 6.3851056) 
(89900, 22.163261) 
(90900, 22.176094) 
(91900, 15.138289) 
(92900, 9.8750925) 
(93900, 15.302319) 
(94900, 28.19075) 
(95900, 23.174503) 
(96900, 9.539457) 
(97900, 22.828949) 
(98900, 12.525942) 
(99900, 12.425152) 
};

==> data/sweet_w_avg_03_00.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, 77.26393) 
(11900, 75.293686) 
(12900, 72.655655) 
(13900, 70.1602) 
(14900, 67.43173) 
(15900, 64.43793) 
(16900, 61.20223) 
(17900, 57.660545) 
(18900, 53.935856) 
(19900, 49.940434) 
(20900, 45.730804) 
(21900, 41.331436) 
(22900, 36.733585) 
(23900, 32.38118) 
(24900, 28.26152) 
(25900, 24.17439) 
(26900, 19.90365) 
(27900, 15.407541) 
(28900, 10.735993) 
(29900, 5.8978953) 
(30900, 0.98901737) 
(31900, -3.9496026) 
(32900, -8.979384) 
(33900, -14.101867) 
(34900, -19.26797) 
(35900, -24.479563) 
(36900, -29.698053) 
(37900, -34.972725) 
(38900, -40.29856) 
(39900, -45.73996) 
(40900, -51.284443) 
(41900, -56.937607) 
(42900, -62.641926) 
(43900, -68.38976) 
(44900, -74.19392) 
(45900, -80.03402) 
(46900, -85.920425) 
(47900, -91.873314) 
(48900, -97.867584) 
(49900, -103.91474) 
(50900, -110.03099) 
(51900, -116.24207) 
(52900, -122.50097) 
(53900, -128.77747) 
(54900, -135.07599) 
(55900, -141.42134) 
(56900, -147.8119) 
(57900, -154.21465) 
(58900, -160.6311) 
(59900, -167.06956) 
(60900, -173.54266) 
(61900, -180.05472) 
(62900, -186.60866) 
(63900, -193.21967) 
(64900, -199.84148) 
(65900, -206.47401) 
(66900, -213.12593) 
(67900, -219.77608) 
(68900, -226.43553) 
(69900, -233.08983) 
(70900, -239.75864) 
(71900, -246.44086) 
(72900, -253.12053) 
(73900, -259.81018) 
(74900, -266.51367) 
(75900, -273.20282) 
(76900, -279.88522) 
(77900, -286.5695) 
(78900, -293.2569) 
(79900, -299.974) 
(80900, -306.7291) 
(81900, -313.51022) 
(82900, -320.3136) 
(83900, -327.14313) 
(84900, -333.99716) 
(85900, -340.8747) 
(86900, -347.79132) 
(87900, -354.75266) 
(88900, -361.75842) 
(89900, -368.7995) 
(90900, -375.87988) 
(91900, -382.99524) 
(92900, -390.13342) 
(93900, -397.31036) 
(94900, -404.51953) 
(95900, -411.7517) 
(96900, -419.02094) 
(97900, -426.31372) 
(98900, -433.63126) 
(99900, -440.96072) 
};

==> data/sweet_w_avg_03_10.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, 776.645) 
(11900, 800.0456) 
(12900, 822.01526) 
(13900, 844.40753) 
(14900, 866.63916) 
(15900, 888.0167) 
(16900, 908.6019) 
(17900, 928.2292) 
(18900, 947.0615) 
(19900, 965.32135) 
(20900, 982.8917) 
(21900, 999.7752) 
(22900, 1016.07764) 
(23900, 1032.3193) 
(24900, 1047.9702) 
(25900, 1063.0819) 
(26900, 1077.5406) 
(27900, 1091.5) 
(28900, 1105.1467) 
(29900, 1118.5298) 
(30900, 1131.6177) 
(31900, 1144.5378) 
(32900, 1157.2212) 
(33900, 1169.7158) 
(34900, 1182.1146) 
(35900, 1194.3934) 
(36900, 1206.5712) 
(37900, 1218.5974) 
(38900, 1230.4994) 
(39900, 1242.2981) 
(40900, 1254.0255) 
(41900, 1265.6309) 
(42900, 1277.128) 
(43900, 1288.5398) 
(44900, 1299.8656) 
(45900, 1311.1025) 
(46900, 1322.2612) 
(47900, 1333.3008) 
(48900, 1344.2295) 
(49900, 1355.0299) 
(50900, 1365.6897) 
(51900, 1376.176) 
(52900, 1386.5071) 
(53900, 1396.6893) 
(54900, 1406.7142) 
(55900, 1416.6608) 
(56900, 1426.5204) 
(57900, 1436.2959) 
(58900, 1445.9655) 
(59900, 1455.5769) 
(60900, 1465.1589) 
(61900, 1474.6512) 
(62900, 1484.0742) 
(63900, 1493.4359) 
(64900, 1502.7352) 
(65900, 1511.9823) 
(66900, 1521.1589) 
(67900, 1530.2697) 
(68900, 1539.3367) 
(69900, 1548.3547) 
(70900, 1557.3099) 
(71900, 1566.222) 
(72900, 1575.0676) 
(73900, 1583.8319) 
(74900, 1592.5278) 
(75900, 1601.1863) 
(76900, 1609.7892) 
(77900, 1618.3206) 
(78900, 1626.7974) 
(79900, 1635.2157) 
(80900, 1643.546) 
(81900, 1651.8204) 
(82900, 1660.0787) 
(83900, 1668.3029) 
(84900, 1676.5045) 
(85900, 1684.657) 
(86900, 1692.751) 
(87900, 1700.7758) 
(88900, 1708.7369) 
(89900, 1716.6593) 
(90900, 1724.5366) 
(91900, 1732.3752) 
(92900, 1740.1586) 
(93900, 1747.8651) 
(94900, 1755.5157) 
(95900, 1763.1431) 
(96900, 1770.725) 
(97900, 1778.2933) 
(98900, 1785.8038) 
(99900, 1793.2848) 
};

==> data/sweet_w_avg_03_20.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, 660.0155) 
(11900, 680.121) 
(12900, 699.0264) 
(13900, 717.4247) 
(14900, 735.29736) 
(15900, 752.772) 
(16900, 769.67834) 
(17900, 785.8649) 
(18900, 801.5863) 
(19900, 816.87604) 
(20900, 831.7395) 
(21900, 846.3105) 
(22900, 860.5111) 
(23900, 874.7296) 
(24900, 888.07336) 
(25900, 900.7917) 
(26900, 912.9166) 
(27900, 924.47614) 
(28900, 935.5761) 
(29900, 946.20776) 
(30900, 956.42456) 
(31900, 966.2456) 
(32900, 975.6388) 
(33900, 984.7021) 
(34900, 993.44934) 
(35900, 1001.9434) 
(36900, 1010.25793) 
(37900, 1018.41174) 
(38900, 1026.4414) 
(39900, 1034.3035) 
(40900, 1042.0503) 
(41900, 1049.6796) 
(42900, 1057.2303) 
(43900, 1064.6389) 
(44900, 1071.896) 
(45900, 1079.0867) 
(46900, 1086.1794) 
(47900, 1093.1578) 
(48900, 1100.0486) 
(49900, 1106.8717) 
(50900, 1113.6661) 
(51900, 1120.3807) 
(52900, 1127.0723) 
(53900, 1133.6691) 
(54900, 1140.2101) 
(55900, 1146.6987) 
(56900, 1153.1643) 
(57900, 1159.556) 
(58900, 1165.897) 
(59900, 1172.1686) 
(60900, 1178.3765) 
(61900, 1184.5094) 
(62900, 1190.5605) 
(63900, 1196.5132) 
(64900, 1202.4218) 
(65900, 1208.3284) 
(66900, 1214.1833) 
(67900, 1219.9928) 
(68900, 1225.7864) 
(69900, 1231.5573) 
(70900, 1237.2697) 
(71900, 1242.9656) 
(72900, 1248.6289) 
(73900, 1254.3159) 
(74900, 1259.972) 
(75900, 1265.6293) 
(76900, 1271.245) 
(77900, 1276.8398) 
(78900, 1282.3655) 
(79900, 1287.8774) 
(80900, 1293.301) 
(81900, 1298.71) 
(82900, 1304.0898) 
(83900, 1309.401) 
(84900, 1314.6943) 
(85900, 1319.9993) 
(86900, 1325.264) 
(87900, 1330.4933) 
(88900, 1335.6879) 
(89900, 1340.8651) 
(90900, 1345.9388) 
(91900, 1350.9722) 
(92900, 1355.969) 
(93900, 1360.9077) 
(94900, 1365.8047) 
(95900, 1370.6279) 
(96900, 1375.373) 
(97900, 1380.0602) 
(98900, 1384.7311) 
(99900, 1389.3892) 
};

==> data/sweet_w_avg_08_00.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, 305.10358) 
(11900, 301.55716) 
(12900, 294.75302) 
(13900, 287.7471) 
(14900, 280.2427) 
(15900, 273.12518) 
(16900, 267.951) 
(17900, 263.32886) 
(18900, 259.45218) 
(19900, 255.76616) 
(20900, 252.92494) 
(21900, 250.4092) 
(22900, 248.01508) 
(23900, 245.71425) 
(24900, 244.01373) 
(25900, 243.96957) 
(26900, 244.71445) 
(27900, 245.97684) 
(28900, 247.3191) 
(29900, 248.83302) 
(30900, 250.25172) 
(31900, 251.6104) 
(32900, 252.7173) 
(33900, 253.54686) 
(34900, 253.9672) 
(35900, 254.54112) 
(36900, 255.27538) 
(37900, 255.92586) 
(38900, 256.35953) 
(39900, 256.84055) 
(40900, 257.6052) 
(41900, 258.5699) 
(42900, 259.82986) 
(43900, 261.1336) 
(44900, 262.56314) 
(45900, 264.02057) 
(46900, 265.3626) 
(47900, 266.63446) 
(48900, 267.90088) 
(49900, 269.08627) 
(50900, 270.0589) 
(51900, 270.78534) 
(52900, 271.42548) 
(53900, 271.79776) 
(54900, 272.00424) 
(55900, 272.06454) 
(56900, 272.0923) 
(57900, 272.05215) 
(58900, 271.98602) 
(59900, 271.6929) 
(60900, 271.24222) 
(61900, 270.8563) 
(62900, 270.60126) 
(63900, 270.51004) 
(64900, 270.44922) 
(65900, 270.359) 
(66900, 270.30957) 
(67900, 270.3534) 
(68900, 270.445) 
(69900, 270.6883) 
(70900, 270.88678) 
(71900, 271.06543) 
(72900, 271.13907) 
(73900, 271.2896) 
(74900, 271.4942) 
(75900, 271.72498) 
(76900, 271.9545) 
(77900, 272.23868) 
(78900, 272.58917) 
(79900, 272.93982) 
(80900, 273.33075) 
(81900, 273.65448) 
(82900, 273.9714) 
(83900, 274.33008) 
(84900, 274.76685) 
(85900, 275.22504) 
(86900, 275.7574) 
(87900, 276.26538) 
(88900, 276.91772) 
(89900, 277.62674) 
(90900, 278.34378) 
(91900, 279.04495) 
(92900, 279.70154) 
(93900, 280.30508) 
(94900, 280.83615) 
(95900, 281.32608) 
(96900, 281.71432) 
(97900, 282.0668) 
(98900, 282.4834) 
(99900, 282.98425) 
};

==> data/sweet_w_avg_08_10.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, -179.10199) 
(11900, -179.92705) 
(12900, -178.2159) 
(13900, -175.28864) 
(14900, -172.36334) 
(15900, -168.4284) 
(16900, -164.35454) 
(17900, -159.4725) 
(18900, -154.74661) 
(19900, -150.90984) 
(20900, -147.71754) 
(21900, -144.47862) 
(22900, -141.19975) 
(23900, -137.60883) 
(24900, -135.25424) 
(25900, -133.35501) 
(26900, -131.90442) 
(27900, -131.10858) 
(28900, -130.56787) 
(29900, -131.25027) 
(30900, -132.23083) 
(31900, -133.29276) 
(32900, -134.17165) 
(33900, -135.26675) 
(34900, -136.45274) 
(35900, -137.74895) 
(36900, -138.92566) 
(37900, -139.81747) 
(38900, -140.6271) 
(39900, -141.07402) 
(40900, -141.43672) 
(41900, -141.71461) 
(42900, -142.21066) 
(43900, -142.67545) 
(44900, -143.23338) 
(45900, -143.91176) 
(46900, -144.78917) 
(47900, -145.8397) 
(48900, -146.81807) 
(49900, -147.59042) 
(50900, -148.2073) 
(51900, -148.79898) 
(52900, -149.52788) 
(53900, -150.33047) 
(54900, -151.12282) 
(55900, -151.92143) 
(56900, -152.73932) 
(57900, -153.51244) 
(58900, -154.36374) 
(59900, -155.24887) 
(60900, -156.31555) 
(61900, -157.40004) 
(62900, -158.40453) 
(63900, -159.4745) 
(64900, -160.39905) 
(65900, -161.11777) 
(66900, -161.87186) 
(67900, -162.7634) 
(68900, -163.71452) 
(69900, -164.6005) 
(70900, -165.53345) 
(71900, -166.46648) 
(72900, -167.43542) 
(73900, -168.47723) 
(74900, -169.40189) 
(75900, -170.25772) 
(76900, -171.13477) 
(77900, -172.00887) 
(78900, -172.78151) 
(79900, -173.43286) 
(80900, -173.95288) 
(81900, -174.45886) 
(82900, -175.00392) 
(83900, -175.56459) 
(84900, -175.95071) 
(85900, -176.21387) 
(86900, -176.41061) 
(87900, -176.57747) 
(88900, -176.64038) 
(89900, -176.71695) 
(90900, -176.75673) 
(91900, -176.9142) 
(92900, -177.15013) 
(93900, -177.41548) 
(94900, -177.73758) 
(95900, -178.09592) 
(96900, -178.49408) 
(97900, -178.91385) 
(98900, -179.24535) 
(99900, -179.45132) 
};

==> data/sweet_w_avg_08_20.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, 109.93582) 
(11900, 104.28809) 
(12900, 99.693214) 
(13900, 95.751274) 
(14900, 93.26247) 
(15900, 95.19812) 
(16900, 98.41234) 
(17900, 101.74461) 
(18900, 105.4168) 
(19900, 108.2422) 
(20900, 110.396996) 
(21900, 112.39041) 
(22900, 113.500694) 
(23900, 115.38882) 
(24900, 117.21121) 
(25900, 118.78764) 
(26900, 119.59214) 
(27900, 120.99117) 
(28900, 123.07312) 
(29900, 126.45808) 
(30900, 130.24231) 
(31900, 133.91121) 
(32900, 137.64012) 
(33900, 141.4237) 
(34900, 144.72156) 
(35900, 147.49907) 
(36900, 150.14243) 
(37900, 152.82675) 
(38900, 155.55733) 
(39900, 158.0196) 
(40900, 160.07283) 
(41900, 161.87859) 
(42900, 163.58182) 
(43900, 164.90916) 
(44900, 165.95822) 
(45900, 167.0187) 
(46900, 168.2939) 
(47900, 169.83647) 
(48900, 171.37782) 
(49900, 172.71593) 
(50900, 174.11745) 
(51900, 175.5165) 
(52900, 176.81569) 
(53900, 178.0333) 
(54900, 179.20795) 
(55900, 180.48575) 
(56900, 181.88179) 
(57900, 183.32138) 
(58900, 184.93481) 
(59900, 186.49182) 
(60900, 187.90929) 
(61900, 189.17299) 
(62900, 190.30925) 
(63900, 191.15427) 
(64900, 191.96443) 
(65900, 192.89499) 
(66900, 193.88235) 
(67900, 194.98471) 
(68900, 195.941) 
(69900, 196.7076) 
(70900, 197.21646) 
(71900, 197.63223) 
(72900, 198.0413) 
(73900, 198.4257) 
(74900, 198.7552) 
(75900, 199.06094) 
(76900, 199.48062) 
(77900, 199.99951) 
(78900, 200.54024) 
(79900, 201.07164) 
(80900, 201.54877) 
(81900, 202.00185) 
(82900, 202.58803) 
(83900, 203.10497) 
(84900, 203.57881) 
(85900, 204.16148) 
(86900, 204.8358) 
(87900, 205.4727) 
(88900, 206.0747) 
(89900, 206.71837) 
(90900, 207.30618) 
(91900, 207.86745) 
(92900, 208.27972) 
(93900, 208.64156) 
(94900, 209.03297) 
(95900, 209.39209) 
(96900, 209.69942) 
(97900, 209.97203) 
(98900, 210.22133) 
(99900, 210.46088) 
};

==> data/sweet_w_avg_24_00.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, -50.65048) 
(11900, -44.79018) 
(12900, -42.81534) 
(13900, -47.29788) 
(14900, -46.135406) 
(15900, -42.719723) 
(16900, -38.38395) 
(17900, -36.474884) 
(18900, -36.11465) 
(19900, -35.01616) 
(20900, -32.332687) 
(21900, -31.130112) 
(22900, -30.455313) 
(23900, -32.159428) 
(24900, -32.782806) 
(25900, -33.18616) 
(26900, -32.91913) 
(27900, -32.274483) 
(28900, -31.709839) 
(29900, -31.528051) 
(30900, -30.918768) 
(31900, -30.888933) 
(32900, -31.053207) 
(33900, -31.03841) 
(34900, -30.1439) 
(35900, -29.083391) 
(36900, -28.708359) 
(37900, -28.37009) 
(38900, -28.011505) 
(39900, -27.742088) 
(40900, -27.5043) 
(41900, -27.020407) 
(42900, -26.793657) 
(43900, -26.627108) 
(44900, -26.409447) 
(45900, -26.089666) 
(46900, -25.784174) 
(47900, -25.389627) 
(48900, -24.895016) 
(49900, -24.666882) 
(50900, -24.122152) 
(51900, -23.77404) 
(52900, -23.20394) 
(53900, -22.865402) 
(54900, -22.467916) 
(55900, -22.320185) 
(56900, -22.119846) 
(57900, -22.09841) 
(58900, -21.900557) 
(59900, -21.749155) 
(60900, -21.583471) 
(61900, -21.442774) 
(62900, -21.044909) 
(63900, -20.966309) 
(64900, -20.781094) 
(65900, -20.416943) 
(66900, -20.035376) 
(67900, -19.781202) 
(68900, -19.4838) 
(69900, -19.331234) 
(70900, -19.300116) 
(71900, -19.071629) 
(72900, -19.06056) 
(73900, -19.11216) 
(74900, -19.107676) 
(75900, -19.127552) 
(76900, -19.060234) 
(77900, -19.09176) 
(78900, -18.985878) 
(79900, -18.8179) 
(80900, -18.663925) 
(81900, -18.61306) 
(82900, -18.535254) 
(83900, -18.433214) 
(84900, -18.297443) 
(85900, -18.094343) 
(86900, -17.944872) 
(87900, -17.741173) 
(88900, -17.530905) 
(89900, -17.376442) 
(90900, -17.351707) 
(91900, -17.32972) 
(92900, -17.325737) 
(93900, -17.251093) 
(94900, -17.222279) 
(95900, -17.220465) 
(96900, -17.200024) 
(97900, -17.378538) 
(98900, -17.324099) 
(99900, -17.379383) 
};

==> data/sweet_w_avg_24_10.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, -4.723237) 
(11900, -9.376735) 
(12900, -8.952327) 
(13900, -9.162202) 
(14900, -8.816877) 
(15900, -6.3593335) 
(16900, -4.5368977) 
(17900, -3.3279624) 
(18900, -2.390324) 
(19900, -0.4089508) 
(20900, 0.00035981) 
(21900, 0.4610853) 
(22900, 0.667046) 
(23900, 2.2324834) 
(24900, 3.1043735) 
(25900, 1.9896626) 
(26900, 2.376867) 
(27900, 2.4249413) 
(28900, 1.9784732) 
(29900, 1.7098068) 
(30900, 1.8797345) 
(31900, 2.1824355) 
(32900, 2.295495) 
(33900, 2.4304423) 
(34900, 2.0990918) 
(35900, 1.9807047) 
(36900, 2.185693) 
(37900, 1.9578115) 
(38900, 1.6877811) 
(39900, 1.2176981) 
(40900, 0.92424613) 
(41900, 0.9717007) 
(42900, 1.0403445) 
(43900, 1.3857449) 
(44900, 1.6088088) 
(45900, 1.5561837) 
(46900, 1.5898203) 
(47900, 1.6957134) 
(48900, 1.6611987) 
(49900, 1.8495681) 
(50900, 1.8351066) 
(51900, 1.9915746) 
(52900, 2.1119905) 
(53900, 2.0312276) 
(54900, 2.2330356) 
(55900, 2.3074439) 
(56900, 2.3754163) 
(57900, 2.4375548) 
(58900, 2.633703) 
(59900, 2.551672) 
(60900, 2.5682425) 
(61900, 2.6128752) 
(62900, 2.7441797) 
(63900, 2.9059913) 
(64900, 3.114044) 
(65900, 3.2865963) 
(66900, 3.411521) 
(67900, 3.4613793) 
(68900, 3.3884454) 
(69900, 3.241008) 
(70900, 3.1243134) 
(71900, 2.7190228) 
(72900, 2.4493115) 
(73900, 2.1412628) 
(74900, 1.9209597) 
(75900, 1.7902027) 
(76900, 1.578116) 
(77900, 1.284518) 
(78900, 1.1396323) 
(79900, 1.0239195) 
(80900, 0.8521791) 
(81900, 0.6785324) 
(82900, 0.41838118) 
(83900, 0.29472086) 
(84900, 0.18399669) 
(85900, 0.03757273) 
(86900, -0.19263287) 
(87900, -0.2902579) 
(88900, -0.41619143) 
(89900, -0.4140542) 
(90900, -0.47948477) 
(91900, -0.4921724) 
(92900, -0.48749948) 
(93900, -0.5975997) 
(94900, -0.67589426) 
(95900, -0.69902945) 
(96900, -0.83267206) 
(97900, -0.9536767) 
(98900, -1.0631795) 
(99900, -1.1609885) 
};

==> data/sweet_w_avg_24_20.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, 48.457905) 
(11900, 38.838097) 
(12900, 29.987244) 
(13900, 30.435175) 
(14900, 30.389437) 
(15900, 31.199411) 
(16900, 33.023808) 
(17900, 34.622467) 
(18900, 34.578297) 
(19900, 33.862045) 
(20900, 32.572636) 
(21900, 31.40844) 
(22900, 30.091352) 
(23900, 31.084976) 
(24900, 31.223999) 
(25900, 30.741426) 
(26900, 28.806942) 
(27900, 27.160107) 
(28900, 26.415014) 
(29900, 25.717926) 
(30900, 25.188484) 
(31900, 24.71606) 
(32900, 24.504187) 
(33900, 24.332497) 
(34900, 24.067116) 
(35900, 23.778345) 
(36900, 24.132385) 
(37900, 24.569853) 
(38900, 24.313322) 
(39900, 23.56027) 
(40900, 22.585617) 
(41900, 21.820312) 
(42900, 21.301329) 
(43900, 20.839024) 
(44900, 20.765587) 
(45900, 20.625164) 
(46900, 20.092733) 
(47900, 19.470959) 
(48900, 19.231417) 
(49900, 18.931086) 
(50900, 18.299667) 
(51900, 17.639645) 
(52900, 17.158022) 
(53900, 16.853174) 
(54900, 16.434666) 
(55900, 16.192503) 
(56900, 15.916174) 
(57900, 15.663244) 
(58900, 15.19749) 
(59900, 14.827544) 
(60900, 14.474645) 
(61900, 14.242221) 
(62900, 14.127696) 
(63900, 13.937942) 
(64900, 13.65543) 
(65900, 13.339917) 
(66900, 13.280079) 
(67900, 13.352196) 
(68900, 13.363189) 
(69900, 13.337765) 
(70900, 13.250548) 
(71900, 12.988324) 
(72900, 12.70797) 
(73900, 12.367167) 
(74900, 12.381849) 
(75900, 12.261089) 
(76900, 11.9268055) 
(77900, 11.716241) 
(78900, 11.353022) 
(79900, 11.191956) 
(80900, 11.160113) 
(81900, 11.293132) 
(82900, 11.373383) 
(83900, 11.253874) 
(84900, 11.209837) 
(85900, 11.302051) 
(86900, 11.2057) 
(87900, 11.048955) 
(88900, 10.738097) 
(89900, 10.670168) 
(90900, 10.642652) 
(91900, 10.61893) 
(92900, 10.45416) 
(93900, 10.400111) 
(94900, 10.333843) 
(95900, 10.153123) 
(96900, 10.0068865) 
(97900, 9.777898) 
(98900, 9.567817) 
(99900, 9.361463) 
};

==> data/sweet_w_avg_31_00.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, 18.938204) 
(11900, 16.699564) 
(12900, 16.465786) 
(13900, 14.507877) 
(14900, 14.533298) 
(15900, 15.727021) 
(16900, 15.875671) 
(17900, 15.744398) 
(18900, 15.093909) 
(19900, 14.496609) 
(20900, 14.608503) 
(21900, 13.984737) 
(22900, 13.212302) 
(23900, 12.543877) 
(24900, 12.53517) 
(25900, 13.13549) 
(26900, 13.026135) 
(27900, 12.773372) 
(28900, 12.922859) 
(29900, 12.871537) 
(30900, 12.849218) 
(31900, 12.890077) 
(32900, 12.709046) 
(33900, 12.59517) 
(34900, 12.51268) 
(35900, 12.398288) 
(36900, 12.412845) 
(37900, 12.30739) 
(38900, 12.31693) 
(39900, 12.276303) 
(40900, 12.389743) 
(41900, 12.335844) 
(42900, 12.327139) 
(43900, 12.43166) 
(44900, 12.301527) 
(45900, 12.480895) 
(46900, 12.357916) 
(47900, 12.195268) 
(48900, 11.919545) 
(49900, 11.909242) 
(50900, 11.998576) 
(51900, 11.889377) 
(52900, 11.701691) 
(53900, 11.856982) 
(54900, 11.953947) 
(55900, 11.834611) 
(56900, 11.792357) 
(57900, 11.639915) 
(58900, 11.342324) 
(59900, 11.111541) 
(60900, 10.874666) 
(61900, 10.822449) 
(62900, 10.670914) 
(63900, 10.611005) 
(64900, 10.360594) 
(65900, 10.276101) 
(66900, 10.156616) 
(67900, 10.05041) 
(68900, 9.930343) 
(69900, 9.631182) 
(70900, 9.4378605) 
(71900, 9.351016) 
(72900, 9.149008) 
(73900, 8.882243) 
(74900, 8.599714) 
(75900, 8.381935) 
(76900, 8.117492) 
(77900, 7.977642) 
(78900, 8.005551) 
(79900, 7.936911) 
(80900, 7.7219896) 
(81900, 7.496792) 
(82900, 7.316829) 
(83900, 7.160244) 
(84900, 6.988309) 
(85900, 6.820087) 
(86900, 6.624961) 
(87900, 6.617845) 
(88900, 6.626376) 
(89900, 6.5402) 
(90900, 6.3715534) 
(91900, 6.2692924) 
(92900, 6.142578) 
(93900, 6.055402) 
(94900, 5.985081) 
(95900, 5.836953) 
(96900, 5.7527804) 
(97900, 5.6230817) 
(98900, 5.554784) 
(99900, 5.4090157) 
};

==> data/sweet_w_avg_31_10.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, -30.692408) 
(11900, -20.663492) 
(12900, -13.646175) 
(13900, -12.993719) 
(14900, -16.060081) 
(15900, -19.147747) 
(16900, -21.275282) 
(17900, -21.681934) 
(18900, -21.648752) 
(19900, -21.516323) 
(20900, -20.831715) 
(21900, -19.443977) 
(22900, -18.766558) 
(23900, -18.264528) 
(24900, -18.659231) 
(25900, -18.487394) 
(26900, -17.410864) 
(27900, -17.400522) 
(28900, -17.665281) 
(29900, -17.265894) 
(30900, -16.91966) 
(31900, -16.39734) 
(32900, -15.967105) 
(33900, -15.1867895) 
(34900, -14.003841) 
(35900, -13.547278) 
(36900, -12.995448) 
(37900, -12.611492) 
(38900, -11.979222) 
(39900, -11.698347) 
(40900, -11.619052) 
(41900, -11.261191) 
(42900, -11.58599) 
(43900, -12.091234) 
(44900, -12.612542) 
(45900, -12.762987) 
(46900, -13.21207) 
(47900, -13.523562) 
(48900, -13.879626) 
(49900, -14.299944) 
(50900, -14.446028) 
(51900, -14.503277) 
(52900, -14.574304) 
(53900, -14.868933) 
(54900, -14.882918) 
(55900, -15.18016) 
(56900, -15.583949) 
(57900, -15.655174) 
(58900, -15.684276) 
(59900, -15.670396) 
(60900, -15.82596) 
(61900, -15.8044615) 
(62900, -15.985279) 
(63900, -16.127573) 
(64900, -16.510954) 
(65900, -16.861597) 
(66900, -17.290852) 
(67900, -17.838692) 
(68900, -18.286936) 
(69900, -18.838093) 
(70900, -19.03897) 
(71900, -19.422781) 
(72900, -19.954512) 
(73900, -20.411358) 
(74900, -20.780497) 
(75900, -21.11475) 
(76900, -21.197432) 
(77900, -21.17934) 
(78900, -21.321606) 
(79900, -21.376175) 
(80900, -21.326656) 
(81900, -21.271364) 
(82900, -21.280918) 
(83900, -21.389778) 
(84900, -21.497818) 
(85900, -21.606144) 
(86900, -21.4712) 
(87900, -21.588223) 
(88900, -21.596926) 
(89900, -21.71387) 
(90900, -21.699863) 
(91900, -21.666504) 
(92900, -21.636618) 
(93900, -21.598665) 
(94900, -21.61314) 
(95900, -21.742702) 
(96900, -21.911718) 
(97900, -21.9805) 
(98900, -22.009035) 
(99900, -22.12248) 
};

==> data/sweet_w_avg_31_20.tex <==
\addplot+[mark=+, thick] coordinates { 
(10900, 31.366074) 
(11900, 26.37305) 
(12900, 24.585337) 
(13900, 28.351004) 
(14900, 30.377304) 
(15900, 29.348835) 
(16900, 29.518145) 
(17900, 28.133) 
(18900, 28.34719) 
(19900, 27.483187) 
(20900, 27.305191) 
(21900, 28.440018) 
(22900, 28.862755) 
(23900, 28.261448) 
(24900, 27.682667) 
(25900, 27.386122) 
(26900, 26.484049) 
(27900, 25.644182) 
(28900, 24.593264) 
(29900, 23.540472) 
(30900, 22.475208) 
(31900, 21.597496) 
(32900, 20.661036) 
(33900, 19.765308) 
(34900, 19.20269) 
(35900, 18.590702) 
(36900, 18.394701) 
(37900, 18.28234) 
(38900, 17.84929) 
(39900, 17.537704) 
(40900, 17.012955) 
(41900, 16.650133) 
(42900, 16.124529) 
(43900, 16.059212) 
(44900, 15.786204) 
(45900, 15.660526) 
(46900, 15.263516) 
(47900, 15.037718) 
(48900, 14.712303) 
(49900, 14.654295) 
(50900, 14.318527) 
(51900, 14.159112) 
(52900, 13.997692) 
(53900, 13.867939) 
(54900, 13.934283) 
(55900, 13.850467) 
(56900, 13.76207) 
(57900, 13.721008) 
(58900, 13.527485) 
(59900, 13.409547) 
(60900, 13.218325) 
(61900, 13.109458) 
(62900, 13.036288) 
(63900, 13.015876) 
(64900, 13.102403) 
(65900, 13.021533) 
(66900, 12.993246) 
(67900, 13.235773) 
(68900, 13.208) 
(69900, 13.116295) 
(70900, 13.074742) 
(71900, 13.0613575) 
(72900, 13.131982) 
(73900, 13.154505) 
(74900, 13.098326) 
(75900, 13.060241) 
(76900, 13.243973) 
(77900, 13.266021) 
(78900, 13.200028) 
(79900, 13.205513) 
(80900, 13.009069) 
(81900, 12.854303) 
(82900, 12.7356615) 
(83900, 12.684776) 
(84900, 12.731992) 
(85900, 12.898275) 
(86900, 13.042705) 
(87900, 13.247372) 
(88900, 13.304591) 
(89900, 13.435091) 
(90900, 13.467224) 
(91900, 13.436685) 
(92900, 13.472025) 
(93900, 13.54537) 
(94900, 13.5988865) 
(95900, 13.730808) 
(96900, 13.773913) 
(97900, 13.700879) 
(98900, 13.717077) 
(99900, 13.661832) 
};

==> noiseless_with_zoom.tex <==
\begin{figure}[h]
  \centering
  \subfloat{\begin{tikzpicture}[spy using outlines={rectangle, yellow,magnification=3, connect spies}]
  \node {\pgfimage[interpolate=true,width=.29\linewidth]{./data/noiseless01000.png}};
 \coordinate (spypoint) at (-1.1, 0.75);
 \coordinate (spyviewer) at (0.8,-0.8);
 \spy[width=2cm,height=2cm] on (spypoint) in node [fill=white] at (spyviewer);
\end{tikzpicture}} \hfill
  \subfloat{\begin{tikzpicture}[spy using outlines={rectangle, yellow,magnification=3, connect spies}]
  \node {\pgfimage[interpolate=true,width=.29\linewidth]{./data/noiseless06000.png}};
 \coordinate (spypoint) at (-1.1, 0.75);
 \coordinate (spyviewer) at (0.8,-0.8);
 \spy[width=2cm,height=2cm] on (spypoint) in node [fill=white] at (spyviewer);
  \end{tikzpicture}} \hfill 
  \subfloat{\begin{tikzpicture}[spy using outlines={rectangle, yellow,magnification=3, connect spies}]
  \node {\pgfimage[interpolate=true,width=.29\linewidth]{./data/noiseless10000.png}};
 \coordinate (spypoint) at (-1.1, 0.75);
 \coordinate (spyviewer) at (0.8,-0.8);
 \spy[width=2cm,height=2cm] on (spypoint) in node [fill=white] at (spyviewer);
  \end{tikzpicture}} \hfill 

  \subfloat[$n = 1000$]{\begin{tikzpicture}[spy using outlines={rectangle, yellow,magnification=3, connect spies}]
  \node {\pgfimage[interpolate=true,width=.29\linewidth]{./data/noise_01000.png}};
 \coordinate (spypoint) at (-1.1, 0.75);
 \coordinate (spyviewer) at (0.8,-0.8);
 \spy[width=2cm,height=2cm] on (spypoint) in node [fill=white] at (spyviewer);
  \end{tikzpicture}} \hfill 
  \subfloat[$n = 6000$]{\begin{tikzpicture}[spy using outlines={rectangle, yellow,magnification=3, connect spies}]
  \node {\pgfimage[interpolate=true,width=.29\linewidth]{./data/noise_06000.png}};
 \coordinate (spypoint) at (-1.1, 0.75);
 \coordinate (spyviewer) at (0.8,-0.8);
 \spy[width=2cm,height=2cm] on (spypoint) in node [fill=white] at (spyviewer);
  \end{tikzpicture}} \hfill 
  \subfloat[$n = 10000$]{\begin{tikzpicture}[spy using outlines={rectangle, yellow,magnification=3, connect spies}]
  \node {\pgfimage[interpolate=true,width=.29\linewidth]{./data/noise_10000.png}};
 \coordinate (spypoint) at (-1.1, 0.75);
 \coordinate (spyviewer) at (0.8,-0.8);
 \spy[width=2cm,height=2cm] on (spypoint) in node [fill=white] at (spyviewer);
  \end{tikzpicture}} \hfill 
\caption{\figuretitle{Noiseless SOUL} On the first row we present three images synthesized during a run of the noiseless
  SOUL methodology. On the second row we present the images obtained at the same iterations for the classical SOUL algorithm.
The initialization are identical and the hyperparameters are fixed as follows: $\delta_n = 10^{-3}$, $\gamma_n = 10^{-5}$ and $m_n = 1$.}
  \label{fig:noiseless}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> ropes.tex <==
\begin{figure}[h]
  \centering
  \subfloat[$m_n = 1$]{\begin{tikzpicture}[spy using outlines={rectangle, yellow,magnification=4, connect spies}]
  \node {\pgfimage[interpolate=true,width=.29\linewidth]{./data/rope_small_langevin_long_iteration.jpg}};
 \coordinate (spypoint) at (-1.1, 0.75);
 \coordinate (spyviewer) at (0.8,-0.8);
 \spy[width=2cm,height=2cm] on (spypoint) in node [fill=white] at (spyviewer);
\end{tikzpicture}} \hfill
  \subfloat[$m_n = 10$]{\begin{tikzpicture}[spy using outlines={rectangle, yellow,magnification=4, connect spies}]
  \node {\pgfimage[interpolate=true,width=.29\linewidth]{./data/rope_middle_langevin_middle_iteration.jpg}};
 \coordinate (spypoint) at (-1.1, 0.75);
 \coordinate (spyviewer) at (0.8,-0.8);
 \spy[width=2cm,height=2cm] on (spypoint) in node [fill=white] at (spyviewer);
  \end{tikzpicture}} \hfill 
  \subfloat[$m_n = 100$]{\begin{tikzpicture}[spy using outlines={rectangle, yellow,magnification=4, connect spies}]
  \node {\pgfimage[interpolate=true,width=.29\linewidth]{./data/rope_long_langevin_small_iteration.jpg}};
 \coordinate (spypoint) at (-1.1, 0.75);
 \coordinate (spyviewer) at (0.8,-0.8);
 \spy[width=2cm,height=2cm] on (spypoint) in node [fill=white] at (spyviewer);
\end{tikzpicture}} \hfill
\label{fig:more_langevin}
\caption{\figuretitle{Langevin iterations and noise} Running the SOUL algorithm with different $m_n$ yield visually coherent images. However the higher $m_n$ is, the noisier the images are. The other hyperparameters are fixed as follow: $\delta_n = 10^{-3}$ and $\gamma_n = 10^{-5}$.}
\end{figure}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

